Bertrand Networks

We study scenarios where multiple sellers of a homogeneous good compete on prices, where each seller can only sell to some subset of the buyers. Crucially, sellers cannot price-discriminate between buyers. We model the structure of the competition by a graph (or hyper-graph), with nodes representing the sellers and edges representing populations of buyers. We study equilibria in the game between the sellers, prove that they always exist, and present various structural, quantitative, and computational results about them. We also analyze the equilibria completely for a few cases. Many questions are left open.

==> multiplicity.tex <==
\subsection{Non-uniqueness of equilibrium}

We present an example demonstrating that there might be multiple equilibria each with a different sketch. This can happen even when the underlying graph is a line, and even restricting ourselves to equilibria in which the support of each seller's price distribution is an interval.  The example demonstrates that a line of length $4$ can admit equilibria with two different sketches.

\paragraph{Example}
\begin{itemize}
\item $4$ sellers, where seller $i$ has captive market of size $\alpha_i$.
\item The sellers are connected in a line, in order of index, with adjacent sellers sharing a market of size $1$.
\item We will choose $(\alpha_1, \alpha_2, \alpha_3, \alpha_4) = (6,3,7,2)$.
\end{itemize}

We note that the unit weight of each shared market is not truly generic.  However, both of the following equilibria continue to exist when the sizes of the shared markets are perturbed by a sufficiently small amount. The parameter values will deform continuously with the magnitude of the perturbation.

For each seller $i$ and each $R_j$ such that $i\in R_j$ we can define $F_{i,j}=F^-_i(t_{j+1})- F^-_i(t_{j})$, and for $R_k$ (the set of sellers with an atom at 1) define $F_{i,k}=1- F^-_i(t_{k})$ to be the size of this atom.


\paragraph{Equilibrium 1}
We define the equilibrium using the notation from the previous section.  We will have $|T|=2$, $t_1 < t_2 < t_3 = 1$.  Our bidding sets are $S_1 = \{3,4\}$, $S_2 = \{2,3\}$, and $S_3 = \{1,3\}$.  (That is, bidders 3 and 4 bid on the range $[t_1,t_2]$, bidders 2 and 3 bid on the range $[t_2, 1]$, and bidders 1 and 3 have atoms at 1).

Solving the linear equations as defined above, our equilibrium is as follows (where all $F_{i,j}$ not listed are assumed to be $0$):
\[ t_1 = \frac{7}{9}, t_2 = \frac{7}{8} \]
\[ F_{1,3} = 1 \]
\[ F_{2,2} = 1 \]
\[ F_{3,1} = \frac{1}{3}, F_{3,2} = \frac{7}{12}, F_{3,3} = \frac{1}{12} \]
\[ F_{4,1} = 1 \]

The functional forms of the price distributions can be solved from these parameters as described above.

\paragraph{Equilibrium 2 (a range common to 3 sellers)}
We now describe a second equilibrium.    We will have $|T|=2$, $t_1 < t_2 < t_3 = 1$.  Our bidding sets are $S_1 = \{3,4\}$, $S_2 = \{1,2,3,4\}$, and $S_3 = \{1,3\}$.

Solving the linear equations as defined above, our equilibrium is as follows:
\[ t_1 = \frac{7}{9}, t_2 = \frac{6}{7} \]
\[ F_{1,2} = \frac{2}{7}, F_{1,3} = \frac{5}{7} \]
\[ F_{2,2} = 1 \]
\[ F_{3,1} = \frac{5}{18}, F_{3,2} = \frac{7}{18}, F_{3,3} = \frac{1}{3} \]
\[ F_{4,1} = \frac{5}{6}, F_{4,2} = \frac{1}{6} \]

The functional forms of the price distributions can be solved from these parameters as described above.


==> pf-thm9.tex <==
\begin{proof} 
The existence of a mixed equilibria in our game follows from the general results of \cite{Simon-Zame}.  They consider
general games where the strategy sets are compact metric spaces and the utility functions are only defined to be continuous on a dense subset
of the space of strategy profiles.  Their main motivation is scenarios where the utilities are continuous everywhere except at 
``tie breaking points'' in which some discontinuity occurs. This is exactly the case we have in our setting where the strategy set of a seller is
exactly the interval $[0,1]$ and the utility of every seller is continuous (linear in his own price) everywhere except at points where 
his price equals that of another seller, in which case a discontinuous jump in utility occurs.  To formally put our setting into their
formalism we simply consider the subspace of strategy profiles that have no ties, which is a dense subset, and over it our utilities are continuous.

The main result of \cite{Simon-Zame} is that as long as we allow our equilibrium to {\em endogenously} choose a ``tie-breaking rule'' 
for the strategy profiles
that lie outside of the dense subset then a mixed Nash equilibrium exists.  Specifically, the endogenously chosen profile of utilities lies in the convex
hull of the utilities in the $\epsilon$-neighbourhoods in the dense subset over which the utility function was exogenously defined and continuous.
In our setting, at a point with a tie between sellers and $i$ and $j$ the endogenously chosen utilities for $i$ and $j$ will be some convex combination
of the utility when $i$ wins the market in case of tie and when $j$ does so, i.e. each of the two players will win a some fraction of the market with the
sum of the fractions being exactly 1.  

At this point we can invoke the fact that, for our games, the tie breaking rule does not matter as discussed in section \ref{tie-breaking}:  For the endogenously chosen tie breaking rule
a mixed Nash equilibrium exists by the results of \cite{Simon-Zame};
this tie breaking rule certainly falls into the family of tie-breaking rules considered in section \ref{tie-breaking} and so
for any other rule in the family the same profile of mixed strategies is still a mixed-Nash equilibrium.
\end{proof}




==> sec-clique.tex <==
\section{Beyond Trees}

In this section we take first steps in going beyond trees, and considering general graphs as the network structure.
Our positive result studies a ``clique'' and identifies an equilibrium with a nice form for it.
We then show that this equilibrium is not unique, however, even for a triangle.  Finally we show that as opposed to the case
of trees, even when there is a single captive market, the equilibrium need not be unique and seller utilities may vary over different
equilibria.


\subsection{Clique}

MOSHE: this result has a bug (triangle with 4,3,2 is a counter example), removed from the paper. 

So the {\em Clique} network we analyze has $n$ sellers, each pair shares a market of size $1$.
Additionally,  each seller $i$ has captive market of size $\alpha_i$, with $\alpha_1 > \alpha_2 > \ldots  > \alpha_n$.

\ignore{

\begin{enumerate}
\item There are $n$ sellers numbered $1 \ldots  n$.
\item Each seller $i$ has captive market of size $\alpha_i$, with $\alpha_1 > \alpha_2 \ldots  > \alpha_n$.
\item Every two sellers share a market of size 1.
\end{enumerate}
}

\begin{theorem}
The following is a sketch solution for an equilibrium of the Clique network:
There are exactly $n$ boundary points $1=t_1 > t_2> \ldots  > t_n > 0$ to be explicitly given below (in the proof body).
The support of each seller $i$ is exactly the interval $[t_{i+1},t_{i-1}]$ (for notational convenience letting $t_0=t_1$ and $t_{n+1}=t_n$).
Seller 1 also has an atom at 1.
The probability that seller $i$ plays below $t_i$ is given by $\Fb_i(t_i)=(t_{i+1}/t_i) \cdot (\alpha_{i+1} + i) - (\alpha_{i+1} + i-1)$.
%Seller utilities are given by $u_i = t_i \cdot (i - 1 + \alpha_i)$,
%\begin{enumerate}
%\item
%The end points of the supports of the sellers are the points $b_0 = b_1 < b_2 < \ldots  < b_n = b_{n+1} = 1$ to be determined below and
%seller $i$'s support is exactly the interval $(b_{i-1},b_{i+1})$.  Seller $n$ will also have an atom at $1$.
%\item
%Seller utilities are given by $u_i = b_i \cdot (n-i + \alpha_i)$.

%On the subrange $(b_{i-1}, b_i)$ we have $F_i(x)=n-i+\alpha_{i-1} - u_{i-1}/x$ (except for seller $1$)
%and in the subrange $(b_i,b_{i+1})$ we have $F_i(x)=n-i+\alpha_{i+1} - u_{i+1}/x$ (except for seller $n$).
%On the subrange $(t_{i+1}, t_i)$ we have $F_i(x)=i+1+\alpha_{i+1} - u_{i+1}/x$ (except for seller $n$)
%and in the subrange $(t_i,b_{i-1})$ we have $F_i(x)=i+1+\alpha_{i-1} - u_{i-1}/x$ (except for seller $1$),
%\end{enumerate}
\end{theorem}

The full form of the distribution functions $F_i$ is
directly implied as described in section \ref{sec:sketches}.

\begin{proof}
We start by describing the process of calculating the boundary points $t_i$ together with the probabilities
$q_i = \Fb_i(t_i)$ and then verify that we get a sketch solution.
%We will have stages $1..n-1$, where at each stage $i$ we will calculate $b_{i+1}/b_i$, as well as $q_{i+1} = 1 - F_{i+1}(b_{i+1})$ (For $i=1$, $q_1 = 1$ and %for $i=n$, $q_n=1-F^-_n(1)$ is the size of the atom at 1).
%After all stages are done, we have $b_n=1$ so we can calculate all the $b_i$'s.  From
%these we calculate the $u_i$'s which finish determining the equilibrium.
We will compute the ratios $t_{i}/t_{i+1}$ starting from $i=n-1$ going down to $i=1$.  After all stages are done we plug $t_1=1$, allowing us
to completely derive the values of all $t_i$.


%\subsubsection{Stage 1}

%At $b_1$, seller $1$ gets all $n-1$ of it competitive markets; while at $b_2$ it gets $n-2$ of them as well as probability $q_2$ of the
%competitive market with seller 2.  At $b_1$, seller $2$ gets all $n-1$ of it competitive markets; while at $b_2$ it gets $n-1$ of them.  So:

%\begin{itemize}
%\item $u_1 = u_1(b_1) = b_1 \cdot (n-1 + \alpha_1)$.
%\item $u_1 = u_1(b_2) = b_2 \cdot (n-2 + q_2 + \alpha_1)$.
%\item $u_2 = u_2(b_1) = b_1 \cdot (n-1 + \alpha_2)$.
%$\item $u_2 = u_2(b_2) = b_2 \cdot (n-2 + \alpha_2)$.
%\end{itemize}

%Dividing the last two equations we get the ratio $b_2/b_1$, and then dividing the first two and plugging the value we have for $b_2/b_1$ we get $q_2$:

%\begin{itemize}
%\item
%$b_2/b_1 = (n-1 + \alpha_2)/(n-2+\alpha_2)$ which is always greater than 1 as needed.
%\item
%$q_2 = (\alpha_2 - \alpha_1)/(n-1+\alpha_2)$ which is always between $0$ and $1$ as needed.
%\end{itemize}

\vspace{0.1in}
\noindent
{\bf Stage $i$:}
\vspace{0.1in}

When pricing at $t_{i+1}$, seller $i+1$ should win exactly the $i$ joint markets with sellers $1,2, \ldots, i$;
while when playing $t_{i}$ he gets the $i-1$ joint markets with $1, 2, \ldots, i-1$ as well as probability $q_{i}$ of the
competitive market with seller $i$.  When pricing at $t_{i+1}$, seller $i$ should win the $i-1$ competitive markets with $1, 2, \ldots,  i-1$
as well as $q_{i+1}$ of its competitive market with $i+1$; while when pricing at $t_{i}$ he wins exactly the $i-1$ competitive markets with $1,2, \ldots,  i-1$.  So
we get the following set of equations:

\begin{enumerate}
\item $u_{i+1} = t_{i+1} \cdot (\alpha_{i+1} + i)$.
\item $u_{i+1} = t_i \cdot (\alpha_{i+1} + i-1 + q_i)$.
\item $u_i = t_{i+1} \cdot (\alpha_i + i-1 + q_{i+1})$.
\item $u_i = t_{i} \cdot (\alpha_i + i-1)$.
\end{enumerate}

The last two equalities, with the value of $q_{i+1}$ we already have from the previous stage (where for the first stage $n-1$, we have $q_n=1$),
allow us to compute:
$$
t_i/t_{i+1} = (\alpha_i + i-1 + q_{i+1})/(\alpha_i + i-1)
$$
which is clearly greater than 1, as long as $q_{i+1}>0$, which we will maintain.  Combining the first two
equations and plugging in $t_i/t_{i+1}$ allows us to compute $q_i$ directly:
$$
q_i = (t_{i+1}/t_i) \cdot (\alpha_{i+1} + i) - (\alpha_{i+1} + i-1)
$$
We now need to ensure that $0 < \Fb_i(t_i)=q_i < 1$. The upper bound is trivial since $t_i > t_{i+1}$.  To prove that $q_i$ is positive it suffices to show
that $t_{i+1} \cdot (\alpha_{i+1} + i) > t_i \cdot (\alpha_{i+1} + i -1)$.   If we look at the function
$f(\alpha) = (\alpha + i)/(\alpha + i - 1)$ then the derivation of $t_i/t_{i+1}$ together with $q_{i+1} \le 1$
gives $t_i/t_{i+1} \le f(\alpha_i)$, where we need to show that $t_i/t_{i+1} < f(\alpha_{i+1})$ which is true since $f$ is strictly decreasing in $\alpha$
and $\alpha_i > \alpha_{i+1}$.




%\begin{itemize}
%\item $u_i = u_i(b_i) = b_i \cdot (n-i + \alpha_i)$.
%\item $u_i = u_i(b_{i+1}) = b_{i+1} \cdot (n-i-1 + q_{i+1} + \alpha_i)$.
%\item $u_{i+1} = u_{i+1}(b_i) = b_i \cdot (n-i-1 + q_i + \alpha_{i+1})$.
%\item $u_{i+1} = u_{i+1}(b_{i+1}) = b_{i+1} \cdot (n-i-1 + \alpha_{i+1})$.
%\end{itemize}

%Dividing the last two equations and plugging in the value we already have for $q_1$,
%we get the ratio $b_{i+1}/b_i$.  Then dividing the first two and plugging
%the value we now have for $b_{i+1}/b_i$ we get $q_{i+1}$:

%\begin{itemize}
%\item
%$b_{i+1}/b_i = (n-i-1 + q_i+ \alpha_{i+1})/(n-i-1+\alpha_{i+1})$ which is always greater than 1 as needed.
%\item
%$q_{i+1} = (\alpha_{i+1}-\alpha_i + q_i (\alpha_i + n-i-1))/(n-i-1 + q_i+\alpha_{i+1})$ which is always between $0$ and $1$, as needed (I think).
%\end{itemize}

\vspace{0.1in}
\noindent
{\bf Verification:}
\vspace{0.1in}

%As $t_1=1$ and we have all the ratios $t_{i+1}/t_i$, we can calculate the values of all $t_i$'s and get the value of all $u_i$'s:
%$u_i = u_i(t_i) = t_{i} \cdot (\alpha_i + i-1)$.

%And then, in the subrange $(b_{i-1}, b_i)$, $F_i$ must make $i-1$ indifferent $u_{i-1} = u_{i-1}(x) = x \cdot (n-i-F_i(x) + \alpha_{i-1})$, while
%in the range $(b_{i}, b_{i+1})$, $F_i$ must make $i+1$ indifferent $u_{i+1} = u_{i+1}(x) = x \cdot (n-i - F_i(x) + \alpha_{i+1})$ so:

%\begin{itemize}
%\item In the subrange $(b_{i-1}, b_i)$: $F_i(x)= n-i+\alpha_{i-1} - u_{i-1}/x$.
%\item In the subrange $(b_{i}, b_{i+1})$: $F_i(x)=n-i+\alpha_{i+1} - u_{i+1}/x$.
%\end{itemize}

%\subsubsection{Verification}

At this point our construction ensured that the $t_i$'s are decreasing as needed, that $1 = \Fb_i(t_{i+1}) > \Fb_i(t_i) = q_i > \Fb_i(t_{i-1}) = 0$ as needed,
and that $u_i(t_{i-1})=u_i(t_i)=u_i(t_{i+1})$ as needed.
%The choice of $b_i$'s and form of the density functions exactly ensure that seller $i$ is indifferent in is range of bidding.
%We need to show that seller $i$ does not want to bid either below or above his range.  Since all density functions are of the form $a-b/x$,
%the utility of $j$ is piece-wise linear.  Thus it suffices to check that $j$ does not desire to bid any $b_i$ for $i>j+1$.
To complete the proof we only need to ensure that for all sellers $i$ and all boundary points $t_j$ we have: $u_i(t_j) \le u_i(t_i)$.  This will be implied
by showing that for $j>i$ we have $u_i(t_{j+1}) \le u_i(t_j)$ while for $j<i$ we have $u_i(t_{j-1}) \le u_i(t_j)$.

For $j<i$ when seller $i$ plays $t_j$ he wins all of his shared markets with sellers $1,2,\ldots,j-1$ as well as $q_j$ of his shared market with $j$, thus
we need to show that $t_{j-1} \cdot (\alpha_i + j-2 + q_{j-1}) = u_i(t_{j-1}) \le u_i(t_j) = t_j \cdot (\alpha_i + j-1 + q_{j})$.  However,
notice that we already know the same inequality with $\alpha_i$ replaced on both sides with $\alpha_j$ (since $u_j(t_{j-1})=u_j(t_j)$ gives
equality without the $q_j$ term on the RHS),
and since $\alpha_j>\alpha_i$ and $t_j < t_{j-1}$ replacing $\alpha_j$ back to $\alpha_i$ reduces the LHS by a larger amount.

Similarly for $j>i$ when seller $i$ plays $t_j$ he wins all shared markets with sellers $1,\ldots,i-1,i+1,\ldots, j-1$ as well as $q_j$ of his shared market with
$j$.  Thus here we need to show $t_{j+1} \cdot (\alpha_i + j-1 + q_{j+1}) = u_i(t_{j+1}) \le u_i(t_j) = t_j \cdot (\alpha_i + j-2 + q_{j})$.  Again,
we have this inequality when we replace $\alpha_i$'s with $\alpha_{j+1}$'s (since $u_{j+1}(t_{j+1})=u_{j+1}(t_j)$ gives equality when
$j-1 + q_{j+1}$ is replaced by the larger $j$), and again this follows for $\alpha_i > \alpha_{j+1}$ since $t_j > t_{j+1}$.


%Let us compare the utilities of seller $j<i$ when playing $b_i$ and $b_{i+1}$.  When playing $b_i$, it wins against sellers $i+1 \ldots  n$ as well as against %seller $i$ with probability $q_i$, so his total utility is $u_j(b_i)=b_i \cdot (n-i+q_i + \alpha_j)$.  Similarly
%$u_j(b_{i+1})=b_{i+1} \cdot (n-i-1+q_{i+1} + \alpha_j)$.  From the first equality we deduce $u_j(b_i) \ge b_i \cdot (n-i + \alpha_j)$ so
%$u_j(b_i)/u_j(b_{i+1}) \ge (b_i/b_{i+1}) \cdot (n-i + \alpha_j)/(n-i-1+q_{i+1} + \alpha_j) \ge
%(b_i/b_{i+1}) \cdot (n-i + \alpha_i)/(n-i-1+q_{i+1} + \alpha_i) = u_i(b_i)/u_i(b_{i+1})=1$.  (The inequality when switching form $\alpha_j$ to
%$\alpha_i$ uses $\alpha_i>\alpha_j$, and the fact that an expression of the form $(a+x)/(b+x)$ with $a\ge b$ is non-increasing in $x$.)  We thus see
%that $u_j(b_j) = u_j(b_{j+1}) \ge u_j(b_{j+2}) \ge \ldots  \ge u_j(b_n)$ as needed to show that $j$ does not want to bid above his range.
%A similar argument should show that $j$ does not want to bid below his range.

\end{proof}

\subsection{Non-uniqueness of equilibrium}

************** TBD -- is this correct? ***********************************

We present a small example demonstrating that the equilibrium described above may not be unique, even in the generic case.

\paragraph{Example}
\begin{itemize}
\item $3$ sellers, where seller $i$ has captive market of size $\alpha_i$, $\alpha_1 < \alpha_2 < \alpha_3$.
\item The sellers are connected in a triangle, where every two sellers share a market of size $1$.
\item We will choose $(\alpha_1, \alpha_2, \alpha_3) = (2,3,4)$.
\end{itemize}

\paragraph{Equilibrium 1 (as described above)}
For this example, there is an equilibrium of the form described in the previous section.  The parameters evaluate as follows:
\[ (b_1, b_2, b_3) = (16/21, 20/21, 1) \]
\[ (u_1, u_2, u_3) = (64/21, 80/21, 4) \]
\[ (q_2, q_3) = (1/5, 17/21) \]
In other words:
\begin{itemize}
\item Seller 1 prices on $[16/21, 20/21]$, with $F_1(16/21) = 0$ and $F_1(20/21)= 1$
\item Seller 2 prices on $[16/21, 1]$ with $F_2(16/21) = 0$, $F_2(20/21) = 4/5$, and $F_2(1) = 1$
\item Seller 3 prices on $[20/21, 1]$ with $F_3(20/21) = 0$, $F_3^-(1) = 4/21$, and prices at exactly $1$ with probability $17/21$.
\end{itemize}
The functional forms of the price distributions can be solved from these parameters as described above.

\paragraph{Equilibrium 2 (a range common to 3 sellers)}
We now describe a second equilibrium.  The form of the equilibrium is as follows, where we have $b_1 < b_2 < 1$.
\begin{itemize}
\item Seller 1 prices on $[b_1,b_2]$, with no atom.
\item Seller 2 prices on $[b_1,1]$ with no atom.  Write $q_2 = 1-F_2(b_2)$.
\item Seller 3 prices on $[b_1,1]$ with an atom at 1.  Write $q_3 = 1-F_3^-(1)$, and $p_3 = 1-F_3(b_2)$.  Note $q_3$ is the size of the atom at $1$.
\end{itemize}
Notably, and unlike in the previous equilibrium, all three sellers price on the range $[b_1, b_2]$.

Write $u_i$ for the utility of seller $i$.  For this to be an equilibrium, the following conditions must hold:
\begin{itemize}
\item $u_1 = b_1(\alpha_1 + 2) = b_2(\alpha_1 + q_2 + p_3)$
\item $u_2 = b_1(\alpha_2 + 2) = b_2(\alpha_2 + p_3) = 1\cdot(\alpha_2 + q_3)$
\item $u_3 = b_1(\alpha_3 + 2) = b_2(\alpha_3 + q_2) = \alpha_3$
\end{itemize}
Setting $(\alpha_1, \alpha_2, \alpha_3) = (2,3,4)$ and solving, we obtain the following solution:
\[ (b_1, b_2) = (2/3, 14/15) \]
\[ (u_1, u_2, u_3) = (8/3, 10/3, 4) \]
\[ q_2=2/7, p_3=4/7, q_3=1/3 \]
In other words:
\begin{itemize}
\item Seller 1 prices on $[2/3, 14/15]$, with $F_1(2/3) = 0$ and $F_1(14/15)= 1$
\item Seller 2 prices on $[2/3, 1]$ with $F_2(2/3) = 0$, $F_2(14/15) = 5/7$, and $F_2(1) = 1$
\item Seller 3 prices on $[2/3, 1]$ with $F_3(2/3) = 0$, $F_3(14/15) = 3/7$, $F_3^-(1) = 2/3$, and prices at exactly $1$ with probability $1/3$.
\end{itemize}
The functional forms of the price distributions can then be solved from these parameters (noting that on the range $[2/3,14/15]$ we have equations for $F_i(x) + F_j(x)$ for each $i \neq j$, from which we can derive a formula for each $F_i(x)$ individually).


==> sketches.tex <==
\subsection{Sketches}
In this section we present some more details about the structure of any equilibrium.
% We show that once one specifies the set of boundary points for the support of each CDF we can compute a unique candidate for an equilibrium, and that it is simple to check if that candidate is indeed an equilibrium.


A {\em  sketch} defines natural number $k$, a list of $k$ points $1=t_1>t_2>\ldots>t_k>0$ which are the {\em transition points}, and sets of sellers $R_1,R_2,\ldots, R_k$ such that for every $j$ it holds that $R_j\neq R_{j+1}$.
Let $T$ be the set of all transition points in the sketch, $T= \{t_1,t_2,\ldots,t_k\}$.
Notation-wise, it would sometimes be convenient to think of the list of points as also including the point $t_{k+1}=0$,
and to think about sets $R_0$ and $R_{k+1}$ which are empty.
Let $\tilde{T}$ be the set of all transition points in the sketch including the additional point we have added,
% Notation-wise, it would sometimes be convenient to think of the list of points as including two additional points $t_0>t_1$ and $0=t_{k+1}<t_k$, and two additional empty sets $R_0$ and $R_{k+1}$.
$\tilde{T}= \{t_1,t_2,\ldots,t_k,t_{k+1}\}$.
Let $T_i\subseteq \tilde{T}$ be the set of transition points for seller $i$, that is, $t_j\in T_i$ if
$i$ is in either $R_{j-1}$ or $R_j$, but not both. % (with the convention that $R_0$ and $R_{k+1}$ are empty). % $i\in R_{j-1} \symdiff R_j$.

We say that CDFs $F_1,F_2,\ldots, F_n$ {\em satisfy a given sketch} if
\begin{itemize}
\item for any seller $i$ and any $j\in \{1,2,\ldots, k-1\}$ such that $i\in R_j$ it holds that the support of $i$ contains $(t_{j+1},t_j)$
\item any seller $i\in R_k$ has an atom at $1$.
\item for each seller $i$, the support of $i$ is exactly the union of the intervals $[t_j,t_{j+1}]$ such that $i\in R_j$.
\end{itemize}

\ignore{
Let $T_i$ be a set of points in $[0,1]$.
We say that $T_i$ is the set of {\em transition points} of CDF $F_i$, if the set $T_i$ is exactly the set of boundary points for $F_i$.
%transition points of $F_i$ the CDF of seller $i$,
Given $T_i$ for each $i$,  let $T=\cup_i^n \ T_i$ be the union of all these sets.
Let $k=|T|$ be the size of $T$.
Assume without lose of generality that these points are ordered in increasing order $1=t_1>t_2>\ldots>t_k\geq 0$.

Given a CDF $F_i$, we say that seller $i$ is {\em pricing on} $(t_j,t_{j+1})$ if $F_i(t_{j+1})> F_i(t_{j})$.
Given CDFs $F_1,F_2,\ldots, F_n$, let $R_j$ denote the set of sellers that are pricing on $(t_j,t_{j+1})$, or equivalently, the set of sellers with support that includes the interval $(t_j,t_{j+1})$.
Note that all sellers that are pricing on that interval are pricing on the entire interval, as none of them has a boundary point in the interval.
We also denote the set of sellers with an atom at $1$ by $R_k$.
}


\begin{lemma}
Assume that we are given an economy and a sketch.
There is a polynomial time algorithm such that if there exists an equilibrium with that sketch then it will compute an equilibrium (a list of CDFs $F_1,F_2,\ldots, F_n$) that satisfies that sketch, and if such an equilibrium does not exists it will provide an evidence to that claim.
Moreover, if there is a unique equilibrium that satisfies that sketch then it can be found by solving a set of linear equation (the general algorithm uses linear program).
\end{lemma}
\begin{proof}
We write a set of linear equations that an equilibrium that satisfies the sketch must satisfy, and show that any solution to the linear program can be used to compute an equilibrium.

It would be useful to denote $y_j(x) = 1-F^-_j(x)$. The variable of the linear program will consist of $u_i$ for every seller $i$, and
$y_j(t)$ for every seller $i$ and $t\in T$ (observe that $t$ itself is not a variable).

% MOSHE: make sure we handle the atom at 1 correctly!

The first type of constraints  states that each seller has the same utility from every price in his support that is transition point.
For any seller $i$ and any $t\in T_i$ we have the equation
\begin{equation}
u_i= t\left(\alpha_i+\sum_{j\in N(i)} \beta_{i,j} \cdot y_j(t)\right)
\end{equation}

The second type of constraints states that each seller has the weakly lower utility by pricing at a transition point that is not his transition point, that is, it is not in the boundary of his support.
For any seller $i$ and any $t\in \tilde{T}\setminus T_i$ we have the equation
\begin{equation}
u_i\geq  t\left(\alpha_i+\sum_{j\in N(i)} \beta_{i,j} \cdot y_j(t)\right)
\end{equation}

The third type of constraints state that the variable indeed make sense for a CDF.
For any seller $i$ and $j\in [k]$ it holds that
\begin{equation}
1\geq y_i(t_j)\geq y_i(t_{j+1})\geq 0
\end{equation}
additionally
% MOSHE: do we need to say $y_i(1)=0$ if $i\notin R_k$, and $y_i(1)>0$ if $i\in R_k$?
%For any seller $i$ and $R_j$ such that $i\notin R_j$ it holds that
\begin{equation}
y_i(0)=1\ \ \forall i
\end{equation}
\begin{equation}
y_i(1)=0\ \ \forall i\notin R_k
\end{equation}
\begin{equation}
y_i(1)>0\ \ \forall i\in R_k
\end{equation}
Note that for $i\in R_k$ the size of the atom of $i$ at $1$ is exactly $y_i(1)$.
% we denote he size of the atom of $i$ at $1$ by $A_i(1) = 1- y_i(1)$.

The fourth type of constraints state that sellers do not price outside their support.
For any seller $i$ and $R_j$ such that $i\notin R_j$ it holds that
\begin{equation}
y_i(t_j)=y_i(t_{j+1})
\end{equation}

Observe that these are indeed a set of linear equations in the variables, and that if there is no solution then no equilibrium that satisfies the sketch exists, as each equation represents some condition that is necessary, either for equilibrium, for the CDFs to be well defined, or for the CDFS to satisfy the sketch.

We next prove that a solution to the equations can be transformed into CDFs that are in equilibrium and satisfies the sketch.
A solution to the linear program specifies $y_i(t)$ for any seller $i$ and $t\in \tilde{T}$. We use the solution to define
$y_j(x) = 1-F^-_j(x)$ for any seller $i$ and $x\in [0,1]$, that coincides with the solution on $\tilde{T}$. 
Together with $F_i(1)=1$ for every $i$, this will completely define a CDF for each seller.

For any seller $i$ and any $j\in [k]$ we define $y_i(\cdot)$ to be a linear function in $1/x$ on the interval $[t_{j+1},t_j]$, that is,
$y_i(\cdot)$ is of the form $y_i(\cdot)= L_{i,j}(x)=a_{i,j}+b_{i,j}/x$.
We fix the linear function to the unique linear function that coincides with the solution at the boundaries, that is
$L_{i,j}(t_{j+1})= y_i(t_{j+1})$ and $L_{i,j}(t_j)=y_i(t_j)$.

Given a solution to the linear program above, for seller $i$ and $t\in \tilde{T}$ define
\begin{equation}
u_i(t) = t\left(\alpha_i+\sum_{j\in N(i)} \beta_{i,j} \cdot y_j(t)\right)
\end{equation}

\ignore{
OLD:

Fix any $x\in (0,1]\setminus T$. There is a unique $j\in [k]$ and a unique $\lambda \in (0,1)$ such that it holds that $x^{-1} = \lambda/t_j + (1-\lambda)/t_{j+1}$.
For any seller $i$ let % we next use the values $y_i(t_j)$ and $y_i(t_{j+1})$ to define the value of $y_i(x)$ as follows
$y_i(x)= \lambda\cdot y_i(t_j) + (1-\lambda)\cdot y_i(t_{j+1})$.
Observe that this completely and uniquely defines a CDF for each seller (when assuming $F_i(1)=1$ for every $i$).
}

The next lemma would be useful.
\begin{lemma}
For the CDFs as defined above, for any seller $i$, and any $j\in [k]$,
the utility $U_i(\cdot)$ is a linear function on the interval $(t_{j+1},t_j)$, moreover, it is the unique linear function that pass through the points $(t_{j+1},u_i(t_{j+1}))$ and  $(t_{j},u_i(t_{j}))$
\end{lemma}
\begin{proof}
Consider any point $x$ in the interval $(t_{j+1},t_j)$.
\begin{equation*}
u_i(x)= x\left(\alpha_i+\sum_{j\in N(i)} \beta_{i,j} \cdot y_j(x)\right)=
x\left(\alpha_i+\sum_{j\in N(i)} \beta_{i,j}  (a_{i,j}+b_{i,j}/x)\right)=
\end{equation*}
\begin{equation*}
x\cdot \alpha_i+\sum_{j\in N(i)} \beta_{i,j} (x\cdot a_{i,j}+b_{i,j})=
\sum_{j\in N(i)} \beta_{i,j} b_{i,j} + x\left(\alpha_i+\sum_{j\in N(i)} \beta_{i,j} a_{i,j}\right)
\end{equation*}
This is clearly a liner function, and clearly it go through the two specified points by the way $y_j(\cdot)$ is defined at these boundary points  for every $j$.
\end{proof}

MOSHE: GOT TILL HERE

This lemma shows that for the defined CDFs it is indeed the case that each $i\in R_j$ is indifferent between all the prices in the interval
$(t_{j+1},t_j)$, and that for any interval $(t_{l+1},t_l)$ such that $i\notin R_l$, $i$ cannot gain by deviating and bidding on that interval. 


%We first observe that the sketch determine the utility of each seller in equilibrium.
FINISH

WE NEED TO PROVE THAT "uniqueness--> WE CAN COMPUTE fast"


\end{proof}


MOSHE: need to define "generic" input, use Lebesgue measure zero.
The next lemma tries to say that for generic input we have uniqueness.
% We say that given economy (specified by a graph and size of captive and shared markets) is {\em generic} if non of the parameters is a solution to any algebraic equation of the others.

MOSHE: need to change the below!
\begin{lemma}
\label{lem:generic-unique}
Assume that we are given an economy and a sketch. If there is an equilibrium that satisfies that sketch then there exist $\delta>0$ such that
with probability $1$ the following economy has a unique equilibrium:
the economy only differ from the original economy by a slight random increase in the size of each captive market. Formally,
a uniformly selected $\epsilon_i\in [0,\delta]$ is added to each $\alpha_i$.
\end{lemma}
\begin{proof}

\end{proof}

\ignore{
\begin{lemma}
Assume that we are given an economy and a sketch. If there is an equilibrium that satisfies that sketch then there exist $\delta>0$ such that
with probability $1$ the following economy has a unique equilibrium:
the economy only differ from the original economy by a slight random increase in the size of each captive market. Formally,
a uniformly selected $\epsilon_i\in [0,\delta]$ is added to each $\alpha_i$.
\end{lemma}
\begin{proof}

\end{proof}
}



OLD :

% There are $n$ sellers and a graph, each two adjacent sellers share a market of size $\beta_{i,j}=1$ .
%Each seller $i\in \{1,2,\ldots,n\}$ has a captive market of mass $\alpha_i>0$.
We consider {\em generic} markets (any market after a minor perturbation).

Consider any equilibrium in this market.
%Let $F_i$ be the CDF of bids for seller $i$, and let $R_i$ be the support of that CDF. Let $u_i$ be the utility of seller $i$ from any bid in his support. A {\em transition point} for seller $i$ is a point $x\in (0,1)$ in which for any small enough $\epsilon>0$, either $F_i(x-\epsilon)=F_i(x)< F_i(x+\epsilon)$ or $F_i(x-\epsilon)<F_i(x)=F_i(x+\epsilon)$. Additionally, $x=1$ is a transition point for $i$, if $i$'s supremum bid is 1. (MOSHE: I am not handling $0$ as we know there is a neighborhood  of $0$ in which no one bids)

Let $T_i$ be the set of transition points of seller $i$, and let $T=\cup_i^n \ T_i$ be the union of all these sets.
Let $t=|T|$.  Assume without lose of generality that these points are ordered in increasing order $t_1<t_2<\ldots<t_t=1$.
We say that seller $i$ is bidding on $(t_j,t_{j+1})$ if $F_i(t_{j+1})> F_i(t_{j})$. Let $R_j$ denote the set of sellers that are bidding on $(t_j,t_{j+1})$. Note that all sellers that are bidding on that interval are bidding on the entire interval. We also denote the set of sellers with an atom at $1$ by $R_t$.

Fix any number of transition points $t$ and fix sets $R_1,R_2,\ldots,R_t$ that are bidding on the intervals.
For any set $R_j$ for $j<t$, consider any agent $i\in R_j$.
It holds that
$$u_i=u_i(t_j)=t_j\left(\alpha_i+\sum_{k\in R_j\setminus \{i\}} (1-F^-_k(t_j))\right)$$
and
$$u_i=u_i(t_{j+1})=t_{j+1}\left(\alpha_i+\sum_{k\in R_j\setminus \{i\}} (1-F^-_k(t_{j+1}))\right)$$

which implies that
$$\frac{t_{j+1}}{t_j}= \frac{\alpha_i+\sum_{k\in R_j\setminus \{i\}} (1-F^-_k(t_j))}{\alpha_i+\sum_{k\in R_j\setminus \{i\}} (1-F^-_k(t_{j+1}))}$$

this holds for $|R_j|$ sellers, which gives us $|R_j|-1$ equations.

For each seller $i$ and each $R_j$ such that $i\in R_j$ we can define $F_{i,j}=F^-_i(t_{j+1})- F^-_i(t_{j})$, and for $R_t$ (the set of sellers with an atom at 1) define $F_{i,t}=1- F^-_i(t_{t})$ to be the size of this atom.

We also know that for every seller $i$ it holds that $F_i(1)=1$, this gives $n$ additional equations.

We can look at all the equations as equations in $F_{i,j}$. The total number of variables in all these equations is $\sum_{j=1}^t |R_j|$.

We conclude that the difference between number of variables an equations is
$\sum_{j=1}^t |R_j| - \sum_{j=1}^{t-1} (|R_j|-1) -n = t-1+|R_t|-n$. As $|R_t|$ is the number of atoms (at 1), for it to be non-negative we need $t\geq n+1-\#atoms$.

% MOSHE:  I now think that the first sum only goes up to $t-1$. This should implies that the difference is actually $|R_j|-t+1-n$.


%This gives us the minimal number of sets in a sketch - there must be at least $t$. Also
Note that any gap in the bid of seller $i$ will result with another equation (saying that utilities on both ends of the gap are the same). So each additional gap implies a need to increase the size of $T$.
For example, if there are only 4 sellers and we want a gap, we need $t\geq 5$.



